CLOTH-HUGS: Cloth Aware Human Gaussian Splatting

We present Cloth-HUGS, a Gaussian Splatting based neural rendering framework for photorealistic clothed human reconstruction that explicitly disentangles body and clothing. Unlike prior methods that absorb clothing into a single body representation and struggle with loose garments and complex deformations, Cloth-HUGS represents the performer using separate Gaussian layers for body and cloth within a shared canonical space. The canonical volume jointly encodes body, cloth, and scene primitives and is deformed through SMPL-driven articulation with learned linear blend skinning weights. To improve cloth realism, we initialize cloth Gaussians from mesh topology and apply physics-inspired constraints, including simulation-consistency, ARAP regularization, and mask supervision. We further introduce a depth-aware multi-pass rendering strategy for robust body-cloth-scene compositing, enabling real-time rendering at over 60 FPS. Experiments on multiple benchmarks show that Cloth-HUGS improves perceptual quality and geometric fidelity over state-of-the-art baselines, reducing LPIPS by up to 28% while producing temporally coherent cloth dynamics.

==> sec_icip/1_intro.tex <==
\section{Introduction}
\label{intro}
% Photorealistic human avatars with controllable pose and clothing dynamics are critical for immersive applications in virtual reality, telepresence, digital fashion, and film production. Recent advances in neural rendering have enabled the creation of high-quality 3D human performers from monocular videos using NeRF-based implicit representations~\cite{mildenhall2020nerf, peng2021neural, weng2022humannerf, noguchi2021neural, su2021anerf, pifuSHNMKL19, jiang2022neuman, peng2021animatable}. These methods typically learn volumetric representations in canonical space and use deformation fields or skeletal-driven transformations to animate the human body. However, they require expensive time and computational costs for both training and rendering, which hinders their applications in real-world scenarios. 


% To address rendering inefficiency, recent research has explored 3D Gaussian Splatting~\cite{kerbl20233d} for real-time neural rendering. Methods like HUGS~\cite{kocabas2023hugs}, GauHuman~\cite{hu2023gauhuman}, and others~\cite{qian2023gaussianavatars, lei2023gart} extend this paradigm to human avatars by combining Gaussians with SMPL-driven deformation~\cite{loper2015smpl}. These methods represent humans with 3D Gaussians in a canonical space, typically initialized from parametric body models, and deform them to posed space through learned Linear Blend Skinning (LBS) weights or deformation fields. They achieve fast training, around 30 minutes, and still maintain high fidelity through adaptive densification strategies and learned appearance models. Although these methods demonstrate impressive speed improvements over NeRF-based approaches, they lack the ability to model cloth as distinct deformable entities. This monolithic representation of body and clothing prevents applications like cloth editing and virtual try-on, while limiting geometric fidelity in loose clothing regions where cloth exhibits independent motion and complex interactions with the body. On the other hand, physics-based cloth simulators~\cite{santesteban2022snug, santesteban2021self, patel2020tailornet, lahner2018deepwrinkles} can generate realistic cloth deformation with accurate cloth-body interactions, wrinkle formation, and physically plausible dynamics. However, integrating their outputs into neural rendering frameworks while maintaining efficient training remains an open challenge.

% Extending Gaussian Splatting to explicit cloth modeling introduces three key challenges. (1) \textit{Cloth-body separation:} distinguishing deformable cloth Gaussians from the body while preserving coherent layering—directly treating cloth as part of the body blurs boundaries and causes motion artifacts. (2) \textit{Physics integration:} Incorporating physics-based priors without losing temporal consistency, as naive simulation-based initialization often breaks under dynamic deformations. (3) \textit{Multi-layer rendering:} handling depth ordering and occlusions between body and cloth layers, which standard single-pass splatting fails to resolve in regions with folds or self-occlusion.


% To tackle these challenges, we propose Cloth-HUGS, a cloth-aware Gaussian Splatting framework with physics-informed optimization that explicitly separates body and cloth representations.
% We construct a canonical Gaussian volume containing distinct layers for body, cloth, and scene primitives. For cloth modeling, we leverage physics simulation (SNUG~\cite{santesteban2022snug}) to introduce cloth-specific Gaussian initialization with topology-aware scales and normal-aligned rotations. 
% To bridge neural rendering with cloth physics, we enforce physics-informed supervision through simulation alignment losses for consistency with simulated geometry, As-Rigid-As-Possible (ARAP) regularization~\cite{sorkine2007rigid} for local shape preservation, and cloth-specific LBS weight regularization derived from simulated meshes that encourages physically plausible skinning, while permitting learned non-rigid refinements. 
% We design a multi-pass rendering pipeline that separately rasterizes body, cloth, and scene layers with depth-aware compositing, efficiently handling complex occlusions. The proposed framework enables photorealistic clothed humans with controllable cloth dynamics, achieving rapid training times (under 40 minutes) while opening novel avenues for cloth editing and virtual try-on.

Photorealistic human avatars with controllable pose and clothing dynamics are fundamental to immersive applications such as virtual reality, telepresence, and digital content creation. NeRF-based human rendering methods reconstruct high-fidelity performers from monocular videos by learning canonical volumetric representations and animating them via deformation fields or skeletal transformations~\cite{mildenhall2020nerf,  weng2022humannerf, jiang2022neuman, peng2021animatable}. Despite impressive quality, their high training and rendering costs limit scalability and practical deployment.

To improve efficiency, recent works adopt 3D Gaussian Splatting~\cite{kerbl20233d} for real-time neural rendering and extend it to humans using SMPL-driven deformation~\cite{loper2015smpl}, achieving fast training while maintaining strong visual fidelity~\cite{kocabas2023hugs, hu2023gauhuman,lei2023gart}. However, these approaches represent clothing and body as a single deformable layer, which restricts geometric expressiveness in loose garments and prevents cloth-specific control such as editing or virtual try-on. In contrast, physics-inspired and simulation-driven garment models provide realistic cloth-body interactions and wrinkle dynamics~\cite{santesteban2022snug, santesteban2021self, patel2020tailornet}, yet integrating such priors into efficient neural rendering remains challenging.

To address these challenges, we propose \textit{Cloth-HUGS}, a cloth-aware Gaussian Splatting framework that explicitly disentangles body and cloth into separate canonical Gaussian layers. We initialize cloth primitives using geometry priors from SNUG~\cite{santesteban2022snug} and refine them with physics-inspired supervision, including simulation-alignment, ARAP regularization~\cite{sorkine2007rigid}, and cloth-specific LBS constraints. Finally, we introduce a depth-aware multi-pass rendering strategy for body-cloth-scene compositing with improved depth ordering. Cloth-HUGS enables photorealistic clothed human synthesis with controllable garment dynamics while retaining rapid training (under 40 minutes).

Our main contributions are as follows:
\begin{itemize}[ topsep=2pt, itemsep=2pt, parsep=0pt, partopsep=0pt]

    \item We propose Cloth-HUGS, which explicitly disentangles body and cloth representations within a 3D Gaussian Splatting representation, enabling physically plausible, high-fidelity cloth deformation and efficient articulation.
    \item We leverage novel physics-guided supervision (including simulation alignment, ARAP, and LBS regularization) and cloth-specific Gaussian initialization to effectively integrate physics-inspired cloth priors, significantly enhancing temporal stability and realism.
    \item A multi-pass, depth-aware rendering pipeline is employed to resolve complex body–cloth–scene occlusions and support seamless compositing, facilitating applications like cloth editing and virtual try-on.
    \item We achieve state-of-the-art results across diverse human motions, resulting in a significant LPIPS reduction (28\% on average in the NeuMan dataset \cite{jiang2022neuman}) and consistent improvement for PSNR, SSIM, and FID, leading to superior perceptual realism and structural fidelity.
\end{itemize}

==> sec_icip/2_related_works.tex <==
% \section{Related Work}
% \label{related_works}
% Neural volumetric representations such as Neural Radiance Fields (NeRF)~\cite{mildenhall2020nerf} have fundamentally transformed novel-view synthesis by jointly encoding scene geometry and appearance within a continuous volumetric field. Although originally designed for static scenes, NeRFs have been extended to dynamic human modeling through learned deformation fields and pose-conditioned radiance representations~\cite{weng2022humannerf,Mubashshira_2025_WACV,jiang2022neuman, guo2023vid2avatar,peng2021animatable}. These approaches achieve remarkable photorealism in animatable human avatars but are computationally demanding, requiring long training times and slow rendering due to the need for volumetric ray integration and per-frame deformation optimization. Furthermore, deformation of implicit fields often relies on complex inverse mappings or root-finding procedures~\cite{chen2021snarf}, which hinder efficiency and scalability. Despite several improvements in acceleration~\cite{chen2022tensorf, reiser2021kilonerf,muller2022instant,fridovich2022plenoxels, liu2020neural}, NeRF-based frameworks remain limited for real-time reconstruction and rendering of articulated humans, motivating the exploration of more explicit and efficient representations.

% To overcome the efficiency and scalability limitations of NeRF-based methods, explicit point-based representations, such as 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d}, have emerged as powerful alternatives that model scenes as collections of anisotropic 3D Gaussian primitives. Each Gaussian encodes position, orientation, opacity, and view-dependent appearance via spherical harmonics, enabling real-time differentiable rendering through rasterization rather than volumetric ray marching. By avoiding costly volumetric integration, 3DGS achieves significantly fast training and inference while maintaining photorealistic quality comparable to NeRF. Subsequent extensions have demonstrated its effectiveness for dynamic and multi-view scenes~\cite{wu20244d, luiten2024dynamic}, showing that explicit Gaussian representations can better capture fine geometric detail and temporal coherence. This paradigm shift from radiance fields to Gaussian primitives provides a compelling foundation for animatable human modeling, combining the interpretability of classical graphics with the flexibility of neural rendering.

% Recent works integrate 3DGS with parametric human body models to efficiently render animatable human avatars. Human Gaussian Splatting (HUGS)~\cite{kocabas2023hugs} learns a disentangled human–scene representation from monocular video by initializing Gaussians with SMPL~\cite{loper2015smpl} and optimizing per-Gaussian Linear Blend Skinning (LBS) weights. Similarly, GauHuman~\cite{hu2023gauhuman} refines SMPL-based weights with a lightweight MLP for fast training and real-time rendering. GaussianAvatars~\cite{qian2023gaussianavatars,zielonka2023drivable} extend this idea to expressive face modeling using morphable head priors.

% Although these methods achieve impressive efficiency and photorealism, they treat clothing and body as a single geometry, limiting accurate cloth details.
% Realistic cloth animation through physics-based simulators produces accurate deformations but at high computational cost. TailorNet \cite{patel2020tailornet} learns pose-dependent cloth deformation from simulation data, while PBNS~\cite{bertiche2020pbns} and SNUG~\cite{santesteban2022snug} incorporate physics-informed objectives to capture dynamic wrinkles and collisions without supervision. Despite their physical realism, these models operate purely on mesh geometry and are not integrated into neural rendering frameworks, limiting their generalization and visual coherence.

% Motivated by these limitations, our work introduces Cloth-HUGS, a cloth-aware Gaussian Splatting framework that explicitly separates body and cloth representations using physics-guided supervision. This enables controllable cloth deformation in neural rendering pipelines for efficient, photorealistic clothed human synthesis.
\section{Related Work}
\label{related_works}
\noindent\textbf{NeRF-based human rendering.}
NeRF~\cite{mildenhall2020nerf} represents geometry and appearance in a continuous radiance field and has been extended to animatable humans via deformation fields and pose-conditioned radiance models~\cite{weng2022humannerf,Mubashshira_2025_WACV,jiang2022neuman,guo2023vid2avatar,peng2021animatable}. Despite high visual fidelity, NeRF-based methods are computationally expensive due to volumetric ray integration and complex deformation mappings, often involving inverse warping or root finding~\cite{chen2021snarf}. While acceleration techniques have been proposed~\cite{chen2022tensorf,reiser2021kilonerf,muller2022instant,fridovich2022plenoxels,liu2020neural}, real-time articulated human rendering remains challenging.

\noindent\textbf{Gaussian Splatting and human avatars.}
3D Gaussian Splatting (3DGS)~\cite{kerbl20233d} replaces volumetric integration with explicit anisotropic Gaussian primitives rendered via rasterization, enabling efficient differentiable rendering with competitive quality. Extensions to dynamic scenes demonstrate strong temporal coherence~\cite{wu20244d,luiten2024dynamic}. Recent works integrate 3DGS with parametric human models for efficient avatar reconstruction: HUGS~\cite{kocabas2023hugs} and GauHuman~\cite{hu2023gauhuman} leverage SMPL-driven deformation for real-time rendering, while GaussianAvatars extend this paradigm to expressive face modeling~\cite{qian2023gaussianavatars,zielonka2023drivable}. More recent approaches explore layered human representations, separating clothing from the body using Gaussian primitives or explicit meshes, including CloCap-GS~\cite{clocapgs}, Wang et al.~\cite{wang_cloth}, and Reloo~\cite{reloo}, highlighting the importance of disentangled modeling for improved garment fidelity.

\noindent\textbf{Learning-based and physics-guided cloth modeling.}
Data-driven garment models predict cloth deformation from pose and shape~\cite{patel2020tailornet}, while physics-inspired methods incorporate constraints for wrinkles and collisions~\cite{santesteban2022snug}. Recent work such as PhysAvatar~\cite{zheng2024physavatar} integrates physical simulation into layered human reconstruction, but relies on mesh-based pipelines and costly optimization. These are not directly compatible with efficient neural rendering frameworks.


Building on these insights, we introduce Cloth-HUGS, a cloth-aware Gaussian Splatting framework that explicitly disentangles body and cloth, incorporating physics-guided
supervision for efficient, photorealistic clothed human synthesis.


